A dynamic copula model for probabilistic forecasting of non-Gaussian multivariate time series

Multivariate time series (MTS) data often include a heterogeneous mix of non-Gaussian distributional features (asymmetry, multimodality, heavy tails) and data types (continuous and discrete variables). Traditional MTS methods based on convenient parametric distributions are typically ill-equipped to model this heterogeneity. Copula models provide an appealing alternative, but present significant obstacles for fully Bayesian inference and probabilistic forecasting. To overcome these challenges, we propose a novel and general strategy for posterior approximation in MTS copula models and apply it to a Gaussian copula built from a dynamic factor model. This framework provides scalable, fully Bayesian inference for cross-sectional and serial dependencies and nonparametrically learns heterogeneous marginal distributions. We validate this approach by establishing posterior consistency and confirm excellent finite-sample performance even under model misspecification using simulated data. We apply our method to crime count and macroeconomic MTS data and find superior probabilistic forecasting performance compared to popular MTS models. These results demonstrate that the proposed method is a versatile, general-purpose utility for probabilistic forecasting of MTS that works well across of range of applications with minimal user input.

==> algorithm_forecasting.tex <==
\begin{algorithm}
\caption{Sampler for $\tilde{p}(\By_{T+1:T+H}\given\By_{1:T})$}
Use Algorithm~\ref{alg:gibbs_sampler} to draw $\Bz_{1:T}\com \Beta_{T}\com \BG\com\BSigma\com\BLambda\com\Bv\sim p\left(\Bz_{1:T}\com \Beta_{1:T}\com\Btheta\given\Bz_{1:T}\in\dcal(\By_{1:T})\right)$\;
Compute $(\BG\com\BSigma\com\BLambda\com\Bv)\mapsto\BD_0$ according to Section~\ref{sec:dgfc_dependence}\;
Compute $(y_{1:T,i}\com z_{1:T\com i})\mapsto \tilde{F}_i$ according to (\ref{eq:ma}) for each $i=1\com 2\com ...\com n$\;
Simulate $\Beta_{T+1:T+H}$ from (\ref{eq:model_factor}), initializing from $\Beta_T$\;
Simulate $\Bx_{T+h}\indep\text{N}_n(\BLambda\Beta_{T+h}\com\text{diag}(\Bv))$ for each $h=1\com2\com...\com H$\;
Compute $\Bz_{T+h}=\BD_0^{-1/2}\Bx_{T+h}$ for each $h=1\com2\com...\com H$\;
Compute $\tilde{y}_{T+h,i}=\tilde{F}_i^{-1}\circ\Phi(z_{T+h,i})$ for each $i=1\com 2\com ...\com n$ and $h=1\com2\com...\com H$.
\label{alg:forecasting}
\end{algorithm}

==> section_model.tex <==
\section{The dynamic factor copula model}\label{sec:dgfc}

Now that we can perform approximate Bayesian inference in a generic Gaussian copula model for stationary multivariate time series, we seek to choose a model configuration that enables straightforward statistical computation and scalable inference for many time series. These requirements leads us to select a dynamic factor model (DFM) for our latent process $p(\Bz_t\given\Bz_{1:t-1}\com\Btheta)$:
\begin{align}
    \Beta_t&=\BG\Beta_{t-1}+\Bepsilon_t,&&\Bepsilon_t\iid\text{N}_k(\Bzero\com\BSigma)\label{eq:model_factor}\\
    \unscaled_t\given\Beta_t&\indep\text{N}_n(\BLambda\Beta_t\com \BV) && \BV=\text{diag}(\Bv)\label{eq:model_unscaled}\\
    \latent_t&=\BD_0^{-1/2}\unscaled_t && \BD_0=\text{diag}\left(\text{var}(\unscaled_{t})\right).\label{eq:model_rescale}
\end{align}
We call our copula model based on this latent process a \textit{dynamic Gaussian factor copula} (DGFC). The static parameters $\{\BG\com\BSigma\com\BLambda\com\Bv\}$ govern the cross-sectional and time series dependence of $\Bz_t$ (and subsequently $\By_t$), and the factor dimension $k \ll n$ is a tuning parameter. The lower-dimensional factor $\Beta_t$ follows a first order vector autoregression (VAR) in (\ref{eq:model_factor}), which is the primary source of time series dependence in the model. These dependencies are determined by the transition matrix $\BG$, which we force to have eigenvalues in the unit circle, thus implying stationarity. The full-dimensional latent vector $\unscaled_t$ inherits dynamics from the factor through the loading matrix $\BLambda$ in (\ref{eq:model_unscaled}). In general $\Bx_t$ will not have unit variance in this setup, so finally we rescale by its \emph{marginal} variances in (\ref{eq:model_rescale}) to end with our usual latent variable $\latent_t$, which marginally (integrating over $\Beta_t$ and $\Bx_t$) follows a mean zero, unit variance Gaussian process. 

Dynamic factor models (DFMs) were introduced by \cite{geweke1977chapter} and are popular in macroeconometrics, where they are used to parsimoniously model large cross-sections of macroeconomic time series using a small number of latent factors \citep{sw2016chapter}. \cite{kn1998restat} introduced the Bayesian analysis of these models, and this work continues with the likes of \cite{aw2000jbes} and \cite{bw2015jbes}, who use Bayesian DFMs to study large financial datasets. For our purposes, the main advantages of the factor model involve scaling and computation. We wish to scale our copula model to multivariate time series with modest-to-large cross-sectional dimension $n$, and the low-dimensional factor structure makes this possible. Secondly, the model enjoys tractable properties can make posterior computation easier and more efficient, as we discuss in Section~\ref{sec:priors}.


%in (\ref{eq:model_factor}, \ref{eq:model_unscaled}) is a linear, Gaussian state space system with a VAR law of motion, so during posterior sampling, we can use standard inference techniques like the Kalman simulation smoother and VAR conjugacy in order to make computation easier and more efficient.

\subsection{Priors and posterior computation}\label{sec:priors}

%We close this section with our prior specification. 

Following the discussion in Section~\ref{sec:erl}, we select priors that enable easy access to $p(\Btheta\given\Bz_{1:T}, \Bz_{1:T}\in\dcal(\By_{1:T}))$. We choose a conditionally conjugate prior $\BG^\tr\com\BSigma\sim\text{MNIW}_{k,k}(d_0\com\BPsi_0\com\overline{\BG}_0^\tr\com\BO^{-1}_0)$ for the VAR parameters in (\ref{eq:model_factor}), and to ensure that this process is stationary, we truncate the prior (and consequently the posterior) so that $\BG$ always has eigenvalues within the unit circle. For the variances $\Bv=[v_1\,v_2\,\cdots\,v_n]^\tr$, we take $v_i^{-1}\sim\text{iid}\,\text{Gamma}(\alpha_0\com\beta_0)$. For the factor loadings $\BLambda=[\lambda_{i,l}]$, we use the multiplicative gamma process prior of \cite{bd2011bka}:
\begin{align}
    \lambda_{i,l}&\indep\text{N}(0\com \phi^{-1}_{i,l}\tau_l^{-1})\\
    \phi_{i,l}&\iid\,\text{Gamma}(\nu_0/2\com\nu_0/2)\\
    \tau_l&=\prod_{h=1}^l\delta_h \quad \begin{array}{l}
        \delta_1\sim\text{Gamma}(a_0\com 1)  \\
          \delta_h\iid\text{Gamma}(b_0\com 1).
    \end{array}
\end{align}
The $\phi_{i,l}$ are local scale parameters, the $\tau_l$ are global scale parameters, and the main advantage of this ordered shrinkage prior is to reduce sensitivity to the choice of factor dimension $k$. We collect these hyperparameters in $\BPhi=[\phi_{i,l}]$ and $\Btau=[\tau_1\,\tau_2\,\cdots\,\tau_k]^\tr$, and we include them in the set of copula parameters $\Btheta=\{\BG\com\BSigma\com\BLambda\com\Bv\com\BPhi\com\Btau\}$ that we estimate. In each of the simulations and applications that follow, we use the same default prior hyperparameters: $d_0=k+1$, $\BPsi_0=\BI_k$, $\overline{\BG}_0=\Bzero$, $\BO_0=\BI_k$, $\alpha_0=1$, $\beta_0=0.3$, $\nu_0=3$, $a_0=2$, $b_0=3$.


All of our prior choices are conditionally conjugate, which enables us to access the rank posterior $p(\Bz_{1:T}\com\Btheta\given\Bz_{1:T}\in\dcal(\By_{1:T}))$ with the pure Gibbs sampler in Algorithm~\ref{alg:gibbs_sampler}. When drawing $(\BG\com\BSigma)$ for instance, we condition on $\Beta_{1:T}$ as if they were observed, meaning we can use standard conjugacy results for VARs \citep{karlsson2013chapter}. Or when drawing the $\Beta_{1:T}$, we recognize that (\ref{eq:model_factor}, \ref{eq:model_unscaled}) is a linear, Gaussian state space system, so conditional on $\Bx_{1:T}$, we can draw $\Beta_{1:T}$ exactly using the Kalman simulation smoother. Another computational advantage of our specification pertains to drawing the $\Bz_{1:T}$. Since $\BV$ in (\ref{eq:model_unscaled}) is diagonal, the $\Bz_{1:T}$ are all conditionally independent given $\Beta_{1:T}$ and $\BLambda$. This means that when implementing the truncated normal draw described in Section~\ref{sec:erl}, we can avoid the large matrix inversion involved in the general case, which improves performance tremendously. 

% Need to revise this to reflec tthe fact that the full algorithm and prior details are moved into appendix

\subsection{Posterior predictive simulation}

A key advantage of our approach is that it induces a (pseudo-)posterior predictive distribution that incorporates uncertainty from the estimation of the $F_i$:
\begin{equation}
    \tilde{p}(\By_{T+1:T+H}\given\By_{1:T})
    =
    \int 
    \underbrace{p(\By_{T+1:T+H}\given F_{1:n}\com\Btheta\com\By_{1:T})}_{(\ref{eq:model_factor}, \ref{eq:model_unscaled}, \ref{eq:model_rescale}, \ref{eq:ts_gauss_link})}
    \underbrace{\tilde{p}(F_{1:n}\com\Btheta\given\By_{1:T})}_{(\ref{eq:pseudo})}
    \,
    \dd 
    F_{1:n}
    \,
    \dd
    \Btheta.
\end{equation}
Given a posterior sample $\{\tilde{F}^{(m)}_{1:n}\com\Btheta^{(m)}\}$, we can simulate our model forward on a per-draw basis to generate a posterior predictive sample $\{\tilde{\By}^{(m)}_{T+1:T+H}\}$, as in Algorithm~\ref{alg:forecasting}. Using this Monte Carlo approximation to the posterior predictive distribution, we can produce and evaluate the full range of point, interval, and density predictions. Note that if we use the basic margin adjustment in (\ref{eq:ma}), all draws $\tilde{F}^{(m)}$ are discrete with support at the sample points, meaning our posterior predictive draws are restricted to the unique values observed in the training dataset, similar to a bootstrap sample. Alternatively, we can use the monotone spline version of the margin adjustment to produce draws $\tilde{F}^{(m)}$ that are properly continuous and generate forecasts with full support. We find that the difference is minimal in large enough datasets.


\input{algorithm_forecasting}


\subsection{Competing methods}\label{sec:other}

%In order to stage a fair comparison, we restrict ourselves to simple, general purpose alternatives that are multivariate, that generate posterior predictive distributions, and that have readily available software. In other words, the ones the average user is most likely to reach for in an initial, exploratory analysis. This narrows the field substantially to two main competitors:

The overall approach that we advocate is to model heterogeneous multivariate time series with the dynamic Gaussian factor copula in Section~\ref{sec:dgfc}, and to do Bayesian inference for this model using the posterior approximation in (\ref{eq:pseudo}). We offer this methodology as a versatile, general-purpose utility for probabilistic time series forecasting that works well across of range of applications with minimal user-intensive tuning. To establish this, we conduct a variety of forecast comparisons on real and simulated data in Sections~\ref{sec:forecastsim} and \ref{sec:applications}. In these comparisons, we pit the DGFC against benchmark competitors that could also be reasonably applied in a broad range of time series scenarios with minimal tuning. As such, we consider the following:
\begin{itemize}
    \item (\textbf{BVAR}) Vector autoregressive (VAR) models are a natural starting point for multivariate time series analysis:
    \begin{align*}
        \By_{t}
        &=
        \Bb_0+\sum\limits_{l=1}^p\BB_l\By_{t-l}+\Bepsilon_t,\quad\Bepsilon_t\iid\text{N}_n(\Bzero\com \BSigma).
    \end{align*}
    %As stated, this model is based on the multivariate normal distribution, and in a Bayesian context the posterior predictive distribution can be heavy-tailed to reflect the uncertainty about the covariance matrix. But either way, every variable is assumed to have the same overall distributional shape (with possibly different locations and scales). 
    The \texttt{BVAR} package \citep{kv2021jss} in the \texttt{R} programming language provides an implementation of the \cite{glp2015restat} approach for estimating Bayesian vector autoregressions (BVARs) with hierarchical shrinkage priors. In this scheme, the coefficients $\BB = [\Bb_0\,\BB_1\,\cdots\,\BB_p]$ and error covariance matrix $\BSigma$ are given a conjugate matrix-normal-inverse-Wishart prior with a ``Minnesota'' structure that shrinks the model configuration toward a random walk for each variable. The tightness of the prior around this model configuration is governed by a hyperparameter $\lambda$ that is jointly estimated. In every application below we use the same default prior settings in the \texttt{BVAR} package; %The \texttt{BVAR} package contains other options, but this is the default;
    %https://onlinelibrary.wiley.com/doi/abs/10.1002/hbm.23456
    \item (\textbf{DLM}) State space models are a popular and flexible class of latent variable time series models where an observed time series $\By_t$ is driven by an unobserved time series $\Bmu_t$ that must be estimated, as in this ``local level'' or ``signal-in-noise'' specification:
    \begin{align}
        \By_t&=\Bmu_t+\Bepsilon_t, &&\Bepsilon_t\iid\text{N}_n(\Bzero\com \BW)\label{eq:measurement}\\
        \Bmu_t&=\Bmu_{t-1}+\Bxi_t,&&\Bxi_t\iid\text{N}_n(\Bzero\com\BV).
    \end{align}
    This and many other dynamic linear models (DLMs) are implemented in the \texttt{dlm} \citep{petris2010jss} and \texttt{KFAS} \citep{helske2017jss} packages in \texttt{R}. The latter also supports dynamic \textit{generalized} linear models (DGLMs) for modeling count-valued data. In this case, the so-called measurement equation in (\ref{eq:measurement}) can be replaced with something like $y_{t,i}\given \mu_{t,i}\sim\text{indep}\,\text{Poisson}(\exp(\mu_{t,i}))$. So the basic DGLM models a multivariate count time series $\By_t$ as a collection of Poisson variables with time-varying parameters that evolve according to a random walk with correlated errors. \texttt{KFAS} also supports count models based on the negative-binomial family. By default the static parameters $\BW$ (when included) and $\BV$ are estimated via maximum likelihood. Since these are full, dense matrices, the DLM is a multivariate model that captures dependence among the $\By_t$.
\end{itemize}

==> table_prior.tex <==
\begin{table}
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Default priors for all simulation exercises and real-data applications}
    \label{tab:priors}
\end{table}
